Universal Cancellations in Uniform Random Waves

A vast literature over the past fifteen years has been devoted to the study of the geometric properties of Gaussian random waves. In this work, we investigate the geometric behavior of \emph{uniform random waves}, a much less studied non-Gaussian model in which the $L^2$ norm is constrained to be exactly equal to one in every realization (a normalization that is natural from the standpoint of quantum mechanics). We show that this norm-constrained formulation has deep consequences for the universality of the so-called \emph{Berry's cancellation phenomenon}, as well as for novel high-frequency asymptotic variance estimates. These effects manifest themselves in both local geometric functionals, such as the Lipschitz--Killing curvatures, and global ones, such as the number of connected components above a fixed threshold. A key byproduct of our analysis is a new explicit relation between Hermite expansions and spherical harmonic decompositions for $0$-homogeneous functionals of Gaussian vectors, which enables a systematic chaos-based analysis of non-Gaussian random waves.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{mathrsfs}
%\parskip4pt plus2pt minus2pt

\usepackage{tikz}
\usepackage{verbatim}
\usetikzlibrary{arrows,shapes}

\usepackage{coffee4}

%% Language and font encodings
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\RequirePackage{etex}%removing this line, on Overleaf, one gets a Warning saying to add this line
\usepackage[T1]{fontenc}
\usepackage{wrapfig}
\usepackage{esint}
%\usepackage{ dsfont }
%% Sets page size and margins
\usepackage[top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}
%\setlength {\marginparwidth }{2cm}

%% Useful packages
\usepackage{physics}%for diagonal matrices ( \mqty[\dmat{1,2,3,4}]) and...? 
\usepackage{amsmath,amssymb}
\renewcommand{\Bbb}{\mathbb}%\Bbb is obsolete and has been renamed \mathbb. Now both works as the latter version
\usepackage{graphicx}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks=true, allcolors=BlueViolet, pagebackref=true]{hyperref}
\renewcommand*\backref[1]{\ifx#1\relax \else (Cited on p.#1) \fi}
\usepackage{cite}
\usepackage[shortlabels]{enumitem}
%https://www.overleaf.com/project/636ccf354d0c7664923ec4fb
%\usepackage{enumerate}%per scegliere il tipo di enumerazione
%\usepackage[all,cmtip]{xy}
%\usepackage{tikz-cd}
%\usepackage{lmodern}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.17}
%\usetikzlibrary{intersections}
%\usepackage{relsize}
\usepackage{subcaption}
\usepackage{dsfont}
\usepackage{cleveref}
%\usepackage{autonum}
%\usepackage{xspace} 
\usepackage{cancel}
%\usepackage{ulem}
%\usepackage{fancyvrb}

%\usepackage[scr=rsfso]{mathalpha} %lettere minuscole belle https://tex.stackexchange.com/questions/575481/like-ell-but-for-j

%frak= Select the fraktur alphabet from euler, lucida, mathpi, mma, mt, esstix, boondox, pxtx, stixtwo.
%sostituisce \mathfrak
%%%%%%%%%%%
%comando\mathbdx{} per scrivere col font BOONDOX, molto calligrafico
%
\DeclareFontFamily{U}{BOONDOX-calo}{\skewchar\font=45 }
\DeclareFontShape{U}{BOONDOX-calo}{m}{n}{
  <-> s*[1.05] BOONDOX-r-calo}{}
\DeclareFontShape{U}{BOONDOX-calo}{b}{n}{
  <-> s*[1.05] BOONDOX-b-calo}{}
\DeclareMathAlphabet{\mathbdx}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathbdx}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbbdx}{U}{BOONDOX-calo}{b}{n}
%%%%%%%%%%%%%%%%%%%%

%%Commands

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{problem}{Problem}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%Per richiamare i teoremi con lo stesso numero
\newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

% Per numerare manualmente definitions and theorem

\newtheorem{manualdefinitioninner}{Definition}
\newenvironment{manualdefinition}[1]{%
  \IfBlankTF{#1}
    {\renewcommand{\themanualdefinitioninner}{\unskip}}
    {\renewcommand\themanualdefinitioninner{#1}}%
  \manualdefinitioninner
}{\endmanualdefinitioninner}

\newtheorem{manualtheoreminner}{Theorem}
\newenvironment{manualtheorem}[1]{%
  \IfBlankTF{#1}
    {\renewcommand{\themanualtheoreminner}{\unskip}}
    {\renewcommand\themanualtheoreminner{#1}}%
  \manualtheoreminner
}{\endmanualtheoreminner}
  
% Per numerare i teoremi con le lettere:
\newtheorem{mainthm}{Theorem}
\renewcommand*{\themainthm}{\Alph{mainthm}}
%
%(https://tex.stackexchange.com/questions/1852/how-to-enumerate-theorems-using-letters) If your counter has the name theorem, the corresponding output command has the name \thetheorem. The command \Alph takes a counter as argument and returns the value converted into the corresponding capital letter. \alph would return lowercase letters instead.
%Quanto è meta?

\theoremstyle{remark} 
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{question}[]{Question}
\newtheorem{ass}{Assumption}

% CLEVEREF
\crefname{equation}{Equation}{Equations}
\crefname{multline}{Equation}{Equations}
\crefname{figure}{Figure}{Figures}
\crefname{question}{Question}{Question}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{innercustomthm}{Theorem}{Theorems}
\crefname{mainthm}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{remark}{Remark}{Remarks}
\crefname{proposition}{Proposition}{Proposition}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{example}{Example}{Examples}
\crefname{claim}{Claim}{Claim}
\crefname{conjecture}{Conjecture}{Conjecture}
\crefname{enumi}{}{}
\crefname{ass}{Assumption}{Assumption}


%%% Louis cmds

\newcommand\Sp{\mathbb{S}}
\newcommand\Imm{\mathrm{Im}}

\newcommand{\enstq}[2]{\left\{#1~\middle|~#2\right\}}
\newcommand\jump{\par\medskip}
\newcommand\quand{\quad\text{and}\quad}
\newcommand\qsothat{\quad\text{so that}\quad}
\newcommand\quor{\quad\text{or}\quad}
\newcommand\qwith{\quad\text{with}\quad}


%%%% for numbering only the equations that we refer to and at the same time for numbering them according to the section they belong to
%\usepackage{mathtools} 
%\mathtoolsset{showonlyrefs,showmanualtags}
\numberwithin{equation}{section}
\usepackage{amsmath}
% \usepackage{showkeys} % scommentare se draft

%%%%% for making comments  -- same colors of the program!
%title frames color
\definecolor{bluola}{RGB}{138,43,226}%blueviolet

\newcommand\commik[1]{(\textbf{\textcolor{bluola}{Mic: #1}})}

\newcommand{\miknew}[1]{{\textcolor{Green}{#1}}}

\newcommand\reftodo[1]{\textbf{\textcolor{WildStrawberry}{[#1]}}}
\newcommand{\repet}[1]{\textcolor{green}{#1}}

%%%%proposed shortcuts
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\cjboh}{\mathfrak{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\P}{\mathbb{P}}
%\newcommand{\dd}{\mathrm{d}}
\newcommand{\der}[1]{\frac{\dd}{\dd #1}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\HX}{\mathcal{H}_X}
\newcommand{\Me}{\mathcal{M}}


\newcommand{\de}{\partial}

\renewcommand{\div}[1]{\mathrm{div}(#1)}
%%letters_v
\newcommand{\f}{\varphi}
\renewcommand{\a}{\alpha}
\newcommand{\e}{\varepsilon}
\newcommand{\w}{\omega}

%Riemannian
\newcommand{\vol}[1]{\mathrm{Vol}^{#1}}
\newcommand{\Vect}{\mathfrak{X}}
\newcommand{\y}{\mathbbm{y}}
\newcommand{\NN}{\frac{N}{\vol{}(M)}}

%\newcommand{\h}{\Vec{\mathrm{H}}}

%\renewcommand{\H}{\mathrm{H}}


%CHAOS
\newcommand{\Var}{{\mathbb{V}\mathrm{ar}}}
\newcommand{\Cov}{\mathrm{Cov}}
%RRW
\newcommand{\berry}{\mathbdx{b}}
\newcommand{\teal}{\color{teal}}

\newtheorem*{theorem*}{\bf Theorem}

%ball and spheres
\newcommand{\uball}{b}
\newcommand{\usph}{s}
% \newcommand{\Sp}{\mathbbm{S}}

%vv \randin from MathiStec code
\def\randin{%
  \mathchoice%
    {\raisebox{-.35ex}{$\displaystyle{^\subset}$}\mkern-11.5mu\raisebox{+.45ex}{$\displaystyle{_\subset}$}}% \displaystyle
    {\mkern+1mu\raisebox{-.27ex}{$\textstyle{^\subset}$}\mkern-11.7mu\raisebox{+.45ex}{$\textstyle{_\subset}$}}% \textstyle
    {\raisebox{.35ex}{$\scriptstyle\subset$}\mkern-14mu\raisebox{-.15ex}{$\scriptstyle\subset$}}% \scriptstyle
    {\raisebox{.3ex}{$\scriptscriptstyle\subset$}\mkern-13.5mu\raisebox{-.10ex}{$\scriptscriptstyle\subset$}}% \scriptscriptstyle
}
%^^ \randin from MathiStec

%vv randto from MathiStec (c'é un % da togliere)
\newcommand{\maschera}{\textcolor{white}{\scalebox{0.3}{$\blacktriangle$}}}
\newcommand*\FlatOmega{
\mathchoice{
\displaystyle{\Omega}\mkern-14mu\raisebox{+.166ex}{$\displaystyle{\maschera}$}
\mkern+7mu\raisebox{+.166ex}{$\displaystyle{\maschera}$}}{
\hbox{$\textstyle{\Omega}$}\mkern-14mu\raisebox{+.166ex}{\hbox{$\textstyle{\maschera}$}}
\mkern+7mu\raisebox{+.166ex}{\hbox{$\textstyle{\maschera}$}}}{
\scriptstyle{\Omega}\mkern-14mu\raisebox{+.13ex}{$\scriptstyle{\maschera}$}
\mkern+5mu\raisebox{+.13ex}{$\scriptstyle{\maschera}$}}{
\scriptscriptstyle{\Omega}\mkern-14mu\raisebox{+.13ex}{$\scriptscriptstyle{\maschera}$}
\mkern+5mu\raisebox{+.13ex}{$\scriptscriptstyle{\maschera}$}}}
\newcommand{\scaledFlatOmega}{{\scalebox{0.8}{$_{\FlatOmega}$}}}
\newcommand*\randto{
\mathchoice{
\raisebox{-.101ex}{$\displaystyle{-}$}\mkern-4.4mu\raisebox{.729ex}
{$\displaystyle{\scaledFlatOmega}$}
\mkern-5.2mu\raisebox{-.101ex}{$\displaystyle\to$}}{
\raisebox{-.101ex}{\hbox{$\textstyle{-}$}}\mkern-4.4mu\raisebox{.729ex}
{\hbox{$\textstyle{\scaledFlatOmega}$}}
\mkern-5.2mu\raisebox{-.101ex}{\hbox{$\textstyle\to$}}}{
\raisebox{-.101ex}{$\scriptstyle{-}$}\mkern-4.4mu\raisebox{.729ex}{$\scriptstyle{\scaledFlatOmega}$}
\mkern-5.2mu\raisebox{-.101ex}{$\scriptstyle\to$}}{
\raisebox{-.101ex}{$\scriptscriptstyle{-}$}\mkern-4.4mu\raisebox{.729ex}
{$\scriptscriptstyle{\scaledFlatOmega}$}
\mkern-5.2mu\raisebox{-.101ex}{$\scriptscriptstyle\to$}}}

%^^ randto from MathiStec

\DeclareMathOperator{\supp}{supp}
%\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Id}{Id}

\newcommand{\seg}{\underline}

%transversality
\newcommand{\transv}{\mathrel{\text{\tpitchfork}}}
\makeatletter
\newcommand{\tpitchfork}{%
  \raise-0.1ex\vbox{
    \baselineskip\z@skip
    \lineskip-.52ex
    \lineskiplimit\maxdimen
    \m@th
    \ialign{##\crcr\hidewidth\smash{$-$}\hidewidth\crcr$\pitchfork$\crcr}
  }%
}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\m}[1]{\mathcal{#1}}
%   Equations
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\bega}{\begin{equation}\begin{aligned}}
\newcommand{\eega}{\end{aligned}\end{equation}}
% graffe
\newcommand{\kop}{\left\{}
\newcommand{\pok}{\right\}}
%tonde
\newcommand{\tyu}{\left(}
\newcommand{\uyt}{\right)}
%quadre
\newcommand{\qwe}{\left[}
\newcommand{\ewq}{\right]}

\newcommand{\new}[1]{\textcolor{bluola}{#1}}
\newcommand{\Mic}[1]{\textcolor{bluola}{\textbf{[Mic: ``#1'']}}}
